Erd\H os--Hajnal problem for $H$-free hypergraphs

This paper deals with the minimum number $m_H(r)$ of edges in an $H$-free graph with the chromatic number more than $r$. We show how bounds on Ramsey and Tur\'an numbers imply bounds on $m_H(r)$.

==> header.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T2A]{fontenc}
%\usepackage[russian]{babel}
\usepackage{babel}

\usepackage{todonotes}

\usepackage[a4paper, margin=1.5cm]{geometry}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{mathrsfs}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=red,
    filecolor=magenta,      
    urlcolor=cyan,
}

%\usepackage{tikz}

\usepackage{microtype}

%\let\Ho\H

\def\lc{\left\lceil}   
\def\rc{\right\rceil}
\def\lf{\left\lfloor}   
\def\rf{\right\rfloor}


\newcommand{\F}{{\mathbb F}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\E}{{\mathcal E}}
\newcommand{\ch}{\operatorname{ch}}
\renewcommand{\C}{{\mathbb C}}
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Re}{\operatorname{Re}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\SL}[2]{\operatorname{SL}_{#1}(#2)}

\newcommand{\Fano}{{\mathscr F}}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\ex}{\mathrm{ex}}
\newcommand{\dd}{{\mathrm d}}

\renewcommand{\phi}{\varphi}
\newcommand{\eps}{\varepsilon}
\newcommand{\id}{{\mathbf 1_1}}

\newtheorem{lemma}{Lemma}
\newtheorem{statement}{Утверждение}
\newtheorem{proposition}{Предложение}
\newtheorem{conjecture}{Гипотеза}
\newtheorem{problem}{Задача}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Определение}
\newtheorem{remark}{Замечание}
\newtheorem{corollary}{Corollary}

\def\fs{\kern 0.5em}

\newcounter{problemcnt}
\newcommand{\pr}
{
    \medskip
    \stepcounter{problemcnt}
    \noindent\textbf{\theproblemcnt.}\fs
}	
% номер со звёздочкой
\newcommand{\prh}
{
    \medskip
    \stepcounter{problemcnt}
    \noindent\textbf{\theproblemcnt*.}\fs
}	
\newcommand{\newproblems}{\setcounter{problemcnt}{0}}

% нумерация пунктов
\newcounter{pun}[problemcnt]
\def\pu{
    \refstepcounter{pun}%
    \noindent\textbf{(\asbuk{pun})}\ 
}
\def\Pu{
    \smallskip
    \refstepcounter{pun}%
    \noindent\textbf{(\asbuk{pun})}%
    \ 
}

\usepackage{graphicx}
\graphicspath{ {./Images/} }

\usepackage{appendix}


==> results/trash.tex <==
\subsection{Тупая оценка}

Покажем сначала, что если в $H$-свободном 3-графе $G$ не более, чем $Cr^{4-\eps}$ рёбер, то он красится в $r$ цветов.

Пусть $V_0 = V(G)$, 
\begin{equation}
    V_i = \{v \in V_{i-1}: \deg_{G[V_{i-1}]} v > Cr^2\},
    \quad
    i \geq 1.
\end{equation}


По индукции легко получить, что при $i \geq 0$ 
\begin{gather}
    E(G[V_i]) \leq Cr^{4-2^i\eps},
    \\
    |V_{i+1}| \leq \frac C3 r^{2-2^i\eps}.
\end{gather}
Второе неравенство очевидно следует из первого,
а переход "--- применение условия на $\ex$.


Положим $N = \lceil\log_2 \frac5{\eps}\rceil$. Тогда в $V_i$ нет вершин при $i \geq N$.

По ЛЛЛ вершины из $V_{i-1} \setminus V_i$ красятся в
$T = \left\lfloor\frac{r}{N}\right\rfloor$ 
цветов: цвет для каждой вершины выбираем из равномерного распределения, каждое событие "--- «данный треугольник одноцветный» имеет вероятность $\frac{N^2}{r^2}$, каждое событие зависимо не более, чем с $3C_ir^2$ другими, 
\begin{equation}
    e\cdot\frac{1}{T^2}\cdot(3C_ir^2 + 1) < 1
\end{equation}
при больших $r$.

Везде константы зависят только от $\eps$, так что при больших $r$ все неравенства работают.






%----------------------------------------------------


В статье~\cite{bohman2010coloring} предлагается определить класс 3-графов $\mathcal F$, для которых
\[
m_F(r) = r^{3+o(1)} \quad F \in \mathcal F.
\]


Предположим, что $F \in \mathcal F$. Тогда рассмотрим гиперграф $H = (V,E)$, на котором достигается.
В нем $|E| = r^{3+o(1)}$. Можно считать, что $|V| = r^{1+o(1)}$.
Тогда для любого $\varepsilon > 0$ выполняется
\[
123
\]

\section{Обобщаем}

Пусть $H=(V,E)$~--- какой-то гиперграф; рассмотрим многочлен от переменных $x_v$, $v\in V$:
\[
F_H(x)=\prod_{e\in E}\left(\sum_{u,v\in e} q_{e,u,v}(x_u-x_v)\right),
\]
где $q_{e,u,v}$~--- свободные переменные. $F_H(x)\neq 0$ по-прежнему означает, что $x$ задаёт правильную раскраску $H$. При этом 
\[
F_H(x)=\sum_{
\substack{u(\cdot),v(\cdot):E\to V\\
u(e),v(e)\in e,\ u(e)\neq v(e)
}}\prod_{e\in E}q_{e,u(e),v(e)}(x_{u(e)}-x_{v(e)}):=\sum_{u(\cdot),v(\cdot)} F_{H,u(\cdot),v(\cdot)}(x).
\]
При этом если коэффициент $[x^c]F_{H,u(\cdot),v(\cdot)}$ не равен нулю для некоторых $u(\cdot),v(\cdot)$, то не равен нулю и $[x^c]F_H(x)$.

В частности, если $H$ двудолен, то существуют $u(\cdot),v(\cdot)$ такие, что граф на множестве рёбер $\{(u(e),v(e))\}_{e\in E}$ двудолен, то \dots, получаем утверждение выше??







%%%%% старая оценка про m_f(r)
Suppose that $G$ is $F$-free 3-graph with $|E(G)| < Cr^q$ that is not $r$-colorable. Let such $r$ be minimal. We divide vertices of $G$ in two sets of <<small>> vertices with degree $< cr^2$ and complementary set of <<big>> vertices:
    \begin{equation}
        V_{small} = \{v \in V(G) \mid \deg v < cr^2\},
    \end{equation}
    \begin{equation}
        V_{big} = V \setminus V_{small} = 
        \{v \in V(G) \mid \deg v \geq cr^2\}.
    \end{equation}
    
    
    We have $|E(V)| \geq \frac 13 \sum_{v \in V_{big}} \deg v \geq  \frac 13 \cdot cr^2 |V_{big}|,$
    so 
    \begin{equation}
        |V_{big}| \leq \frac3c \cdot Сr^{q-2}.
    \end{equation}
    
    By minimality of $r$ we have $|E(G[V_{big}])| \geq C' \cdot r^q$, where $C' = C / 2^q$.      
   
    
    Let $W_i = \{v \in V_{big} \mid e^i cr^2 \leq \deg v \leq e^{i+1}cr^2\}$.
    Since $|E(G)| < Cr^q$, we see that $W_i = \emptyset$ when $e^i > (C/c)r^{q-2}$, that is
    \begin{equation}
        i > (q-2)\ln r + \ln(C/c).
    \end{equation} 
    
    Let $G' = G[V_{big}]$.
    Let $G_i = G[W_i] = G'[W_i]$. By pigeonhole principle there is some $j$ such that
    \begin{equation}
        |E(G_j)| > C' \cdot \frac{r^q}{(q-2)\ln r + \ln(C/c)} > C'' \cdot \frac{r^q}{\ln r}
    \end{equation}
    So we have $|V(G_j)| \cdot e^{j+1}cr^2 > C'' \cdot {r^q}/{\ln r}$.
    Thus
    \begin{equation}
        |V(G_j)| >  C''' \cdot \frac{r^{q-2}} {e^{j+1}\ln r},
    \end{equation}
    where $C''' = C''/c$.
    And by upper bound on Ramsey number we can find an independent set in $G_j$, hence in $G$, of size at least $(V(G_j)/B)^{1/b}$, and if we remove $V(G_j)$ from $G$, we will remove at least
    \begin{equation}\label{eq:edges_removed}
        |V(G_j)/B|^{1/b} \cdot e^j cr^2
        \geq
        \left(
            \frac{C''' r^{q-2}}{Be^{j+1}\ln r}
        \right)^{1/b}
        \cdot
        e^j cr^2
        =
        C''''\cdot
        \frac{r^{(q-2)/b+2}}{\ln^{1/b} r}
    \end{equation}
    edges.
    We are going to show that for 
    \begin{equation}\label{eq:value_of_q}
        q \leq 2 + \frac{b-1/e}{b-1}
    \end{equation}
    the right-hand side of~\eqref{eq:edges_removed} is more than $c'r^{q-1}$.
    That is, we need $r^{q-2 + 2b} > r^{bq-b} \ln r$
    or
    \begin{equation}
        r^{q-2+2b-bq+b} > \ln r.
    \end{equation}
    It is easy to show (e.\,g.\ by taking derivatives) that $r^{1/e} \geq \ln r$.
    So 
    \begin{equation}
        q-2+2b-bq+b\geq \frac 1e
    \end{equation}
    is enough, from which~\eqref{eq:value_of_q} follows.
    
    
    \vspace{2cm}
    
    Let $V_{t} = \{v \in V(G) \mid \deg v > t\}$. 
    From upper bound on Ramsey numbers we got
    \begin{equation}
        \alpha(G[V_t]) \geq |V_t|^{1/b}.
    \end{equation}
    
    We want to find such $t$ that
    \begin{equation}
        |V_t|^{1/b}\cdot t \geq cr^{q-1}.
    \end{equation}
    
    
    
    
\begin{proposition}
    Consider a 3-graph $F$. Let $a,b,A,B$ be numbers such that for all $t \geq 1$ 
    \begin{equation}\label{eq:ramsey_bounds}
        At^{a} \leq R(F,K_t) \leq Bt^{b}.
    \end{equation}
    Then for all $r \geq 1$
    \begin{equation}
        B'r^{\frac{b}{b-1} + 2} \leq
            m_F(r) 
        \leq A'r^{\frac{3a}{a-1}},
    \end{equation}
    where $A'$ is some number which may depend on $F$, and 
    \begin{equation}
        B' = \left(
            \frac{(1-2^{1-b})}
                {2^{\frac{b}{b-1}+b+3}(12e)^{b-1} B \bigl(\frac b{b-1}+2\bigr)^b}
        \right)^{1/(b-1)}
    \end{equation}
\end{proposition}

% We are going to use the following
% \begin{lemma}[Lemma 8 from \cite{kostochka2001chromatic}]\label{lm:kostochka2001}
% Let $0\leq \alpha <1$ and $\beta<1-\alpha$. Let $H$ be a hypergraph with $n$ vertices.
% Suppose that every subhypergraph $P$ of $H$ (including $H$ itself) with $m \geq 2$ vertices has an
% independent set of size at least $cm^\alpha(\ln em)^\beta$ for some constant $c > 0$. Then there 
% is a $d=d(c,\alpha,\beta)>0$ such that 
% \begin{equation}
%     \chi(H)\leqslant dn^{1-\alpha}(\ln en)^{-\beta}.
% \end{equation}
% \end{lemma}
%
%
\begin{proof}%[Proof of Proposition 1]
    First, let us prove the upper bound on $m_F(r)$.
    The lower bound on Ramsey number states that there is an $F$-free 3-graph $G$ with $|V(G)|\geq At^{a}$ and the independence number $\alpha<t$. The chromatic number of $G$ satisfies
    \begin{equation}
        \chi(G) \geq
        \frac{|V(G)|}{\alpha}
        = At^{a-1}.
    \end{equation}
    Moreover, $|E(G)| \leq |V(G)|^{3}/6 = A^3t^{3a}/6$.
    Combining these two inequalities we get
    \begin{equation}
        |E(G)| \leq \frac{A^3t^{3a}}{6} \leq 
        \frac{A^3}{6} \bigl(\chi(G)^{\frac{1}{a-1}}/A\bigr)^{3a} = 
        \frac{A^{3-3a}}{6} \chi(G)^{\frac{3a}{a-1}}.
    \end{equation}
    
    
    
    
    
    
\subsection{Нижняя оценочка}

В статье~\cite{conlon2010hypergraph} доказывается, что
\[
R_3 (4,n) \leq 2^{cn^2\log n}.
\]

\begin{corollary}
\[
m_{K_4^3} (r) \geq cr^3 \sqrt \frac{\log r}{\log \log r} 
\]
\end{corollary}

Рассмотрим 3-граф $H = (V,E)$ без $K_4^3$ и с маленьким $E(H)$. Покрасим его вершины степени менее $cr^2$ в $r/2$ цветов, воспользовавшись стандартным ЛЛЛ-трюком.


Осталось не более $cr \sqrt \frac{\log r}{\log \log r} =: t$ вершин и $r/2$ цветов.
Найдем $\alpha = \alpha (t)$, для которого мы умеем доказывать неравенство 
\[
R_3 (4,\alpha) \leq t.
\]
Заметим, что оценка начала секции позволяет брать 
\[
\alpha = c \sqrt \frac{\log t}{\log \log t} = c \sqrt \frac{\log r}{\log \log r}.  
\]


Таким образом, гарантированно найдется независимое множество размера $\sqrt \frac{\log r}{\log \log r}$.
Тут вот стоит еще обсудить следует ли из этого $\chi \sim V/\alpha$; мне кажется, что скорее да.






\begin{proof}
    Suppose that $G$ is a $F$-free 3-graph with $|E(G)| < Br^3\ln^A r$ that is not $r$-colorable with minimal such $r$. We divide vertices of $G$ in two sets of <<small>> vertices with degree $< cr^2$ and complementary set of <<big>> vertices:
    \begin{equation}
        V_{small} = \{v \in V(G) \mid \deg v < cr^2\},
    \end{equation}
    \begin{equation}
        V_{big} = V \setminus V_{small} = 
        \{v \in V(G) \mid \deg v \geq cr^2\}.
    \end{equation}
    Put $c = 1/12e$, then by Lemma~\ref{lm:3graph-coloring} $G[V_{small}]$ has a proper coloring with $\lceil r/2 \rceil$ colors. It follows that $G[V_{big}]$ cannot be colored with no more than $r/2$ colors.
    Then 
    \begin{equation}\label{eq:egv_big_is_big}
        |E(G[V_{big}])| > \frac{B}{8} \cdot r^3\cdot \ln^A r/2.
    \end{equation}
    
    Let $V_{big} = V_0 \cup V_1 \cup V_2 \cup \dots$, where
    \begin{equation}
        V_k = \{ v \in V(G) \mid 2^k cr^2 \leq \deg v < 2^{k+1}cr^2\}.
    \end{equation}
    
    
    Suppose there is some $k$ for which
    \begin{equation}\label{eq:alphaGVk2}
        \alpha(G[V_k]) \geq \frac{B}{2^{k-1}cr^2}\bigl(r^3\ln^Ar - (r-1)^3\ln^A(r-1)\bigr).
    \end{equation}
    Then we can paint the vertices from a corresponding independent set in one color. Now if we remove colored vertices from $G$, we get a 3-graph with less than 
    \begin{equation}
        Br^{3}\ln^A r - \frac 12 \cdot 2^{k}cr^2\cdot \alpha(G[V_k]) = B(r-1)^{3}\ln^A(r-1)
    \end{equation}
    edges that is not $(r-1)$-colorable. That is a contradiction to the minimality of $r$.
    So we can assume that for every $k$ the contrary of~\eqref{eq:alphaGVk2} holds, so by upper bound from~\eqref{eq:ramsey_exp_bounds} we have
    \begin{equation}
        |V_k| < t^{Ct},\qquad t =
            \frac{B}{2^{k-1}cr^2}\bigl(r^3\ln^Ar - (r-1)^3\ln^A(r-1)\bigr).
    \end{equation} 
    Using the fact that $x^3\ln^A x - (x-1)^3\ln^Ax \leq 4x^2\ln^A x$ for $x \geq 2$, we get
    \begin{equation}
        |V_k| < \left(
            \frac{B}{2^{k-1}c}\cdot \ln^A r\right)^%
                {CB\ln^A r / (2^{k-1}c)}.
    \end{equation}
    Now let $e_k$ be the number of edges that pass through vertices of $V_k$. We have
    \begin{equation}
        |E(G[V_{big}])| < \sum_{k \geq 0} e_k
        < \sum_{k \geq 0} 2^{k+1}cr^2 \cdot 
            \left(
                \frac{B}{2^{k-1}c}\cdot \ln^A r
            \right)^%
            {CB\ln^A r / (2^{k-1}c)}.
    \end{equation}
    Но каждая скобочка ограничена снизу величиной $e^{-C/e}$, 
    а так как $2^kcr^2 < |E|$, то всего слагаемых в плохом случае $\log (r \ln^A r)$, то есть получается оценка снизу
    \begin{equation}
        cr^2 \cdot 2^{k+1} \cdot e^{-C/e}
        =
        C' r^3 \ln^A r,
    \end{equation}
    беда(
    
    ПОПЫТКА БОЛЕЕ ОБЩЕГО РАССУЖДЕНИЯ
    
    
    Let $V_{big} = V_0 \cup V_1 \cup V_2 \cup \dots$, where
    \begin{equation}
        V_k = \{ v \in V(G) \mid a_k(r) cr^2 \leq \deg v < a_{k+1}(r)cr^2\},
    \end{equation}
    where $a_k(r)$ is some sequence of numbers.
    
    Suppose there is some $k$ for which
    \begin{equation}\label{eq:alphaGVk2}
        \alpha(G[V_k]) \geq \frac{2B}{a_k(r)cr^2}\bigl(r^3\ln^Ar - (r-1)^3\ln^A(r-1)\bigr).
    \end{equation}
    Then we can paint the vertices from a corresponding independent set in one color. Now if we remove colored vertices from $G$, we get a 3-graph with less than 
    \begin{equation}
        Br^{3}\ln^A r - \frac 12 \cdot a_k(r)cr^2\cdot \alpha(G[V_k]) = B(r-1)^{3}\ln^A(r-1)
    \end{equation}
    edges that is not $(r-1)$-colorable. That is a contradiction to the minimality of $r$.
    So we can assume that for every $k$ the contrary of~\eqref{eq:alphaGVk2} holds, so by upper bound from~\eqref{eq:ramsey_exp_bounds} we have
    \begin{equation}
        |V_k| < t^{Ct},\qquad t =
            \frac{2B}{a_k(r)cr^2}\bigl(r^3\ln^Ar - (r-1)^3\ln^A(r-1)\bigr).
    \end{equation} 
    Using the fact that $x^3\ln^A x - (x-1)^3\ln^Ax \leq 4x^2\ln^A x$ for $x \geq 2$, we get
    \begin{equation}
        |V_k| < \left(
            \frac{2B}{a_(k)c}\cdot \ln^A r\right)^%
                {2BC\ln^A r / (a_k(r)c)}.
    \end{equation}
    Now let $e_k$ be the number of edges that pass through vertices of $V_k$. We have
    \begin{equation}
        |E(G[V_{big}])| < \sum_{k \geq 0} e_k
        < \sum_{k \geq 0} a_{k+1}(r)cr^2 \cdot 
            \left(
                \frac{2B}{a_k(r)c}\cdot \ln^A r
            \right)^%
            {2BC\ln^A r / (a_k(r)c)}.
    \end{equation}
    Нам нужно неравенство
    \begin{equation}
        \sum_{k \geq 0}^{a_k(r) < Br\ln^A r/c} a_{k+1}(r)
            \left(
                \left(
                    \frac{2B}{a_k(r)c}\cdot \ln^A r
                \right)^%
                    {2B\ln^A r / (a_k(r)c)}
            \right)^C
            \leq
            \frac{B}{8c} \cdot r \ln^A(r/2).
    \end{equation}
    % Combining this with~\eqref{eq:egv_big_is_big} and substituting $C$ and $c$ we get
    % \begin{equation}
    %     \frac{B'}{2^{\frac b{b-1}+2}} < \frac{(1/12e)B{B'}^b\bigl(\frac b{b-1}+2\bigr)^b 2^{b+1}}{(1/12e)^b(1-2^{1-b})} 
    % \end{equation}
    % or
    % \begin{equation}
    %     {B'}^{b-1} < \frac{(1-2^{1-b})}{2^{\frac b{b-1}+b+3} (12e)^{b-1}B\bigl(\frac b{b-1}+2\bigr)^b},
    % \end{equation}
    % that's a contradiction.
\end{proof}

% \subsection{Выводы из точной оценки}
% The following theorem is from~\cite{fox2019independent}:
% \begin{theorem}[Theorem 1.1 from~\cite{fox2019independent}]
% We have $R_3(K_4^{(3)-}, K_t) = t^{\Theta(t)}$.
% \end{theorem}
% Using same arguments as in fist section of proof of Proposition~\ref{pr:abAB}, we obtain the following result.
% \begin{proposition}
% As $r$ tends to infinity,
% \begin{equation}
%     m_{K_4^{(3)-}} (r) \leq r^{3 + o(1)}.
% \end{equation}
% \end{proposition}
% \begin{proof}
% In particular, there is a constant $C$ such that for each $t \geq 1$ there is a graph $G_t$ with $|V(G_t)| = t^{C_t}$ and $\alpha(G_t) < t$. Then
% \begin{equation}
%     \chi(G_t) \geq \frac{|V(G_t)|}{\alpha(G_t)}
%     > t^{Ct - 1}.
% \end{equation}
% Let $(t-1)^{C(t-1) - 1} \leq r < t^{Ct - 1}$.
% \begin{equation}
%     |E(G_t)|
%     < \frac{|V(G_t)|^3}{6}
%     = \frac{t^{3Ct}}{6}
%     = \frac16 (t^{Ct-1})^{\frac{3Ct}{Ct-1}}
%     = \frac16 (t^{Ct-1})^{3+\frac 3{Ct-1}}.
% \end{equation}
% Note that for $t \geq 2$
% \begin{equation}
%     t^{Ct-1} < e^C(t-1)^{Ct- 1},
% \end{equation}
% so
% \begin{equation}
%     |E(G_t)|
%     < 
%     \frac16 (e^C \cdot (t-1)^{Ct-1})^{3+\frac 3{Ct-1}}
%     <
%     \frac16 \cdot e^{C\cdot (3+\frac 3{Ct-1})} \cdot (t-1)^{3+\frac 3{Ct-1}} \cdot r^{3 + \frac 3{Ct-1}}.
% \end{equation}
% As $r$ tends to $+\infty$, so does $t$, and we have
% \begin{equation}
%     \frac16 \cdot e^{C\cdot (3+\frac 3{Ct-1})} = r^{o(1)},
% \end{equation}
% \begin{equation}
%     (t-1)^{3+\frac 3{Ct-1}} 
%     = r^{\log_r(t-1) \cdot (3 + \frac 3{Ct-1})}
%     < r^{\frac 1{C(t-1)-1} \cdot (3 + \frac 3{Ct-1})}
%     = r^{o(1)},
% \end{equation}
% \begin{equation}
%     r^{3+\frac 3{Ct-1}} = r^{3 + o(1)},
% \end{equation}
% so 
% \begin{equation}
%     m_{K_4^{(3)-}}(r) \leq r^{3 + o(1)}.
% \end{equation}
% \end{proof}

% То есть для данного $t$ найдётся $K_4^{(3)-}$-свободный 3-граф $G$ с $\alpha(G) < t$ на $t^{C_1t}$ вершинах.
% Кроме того, если в $K_4^{(3)-}$-свободном 3-графе $G$ будет больше $t^{C_2t}$ вершин, то $\alpha(G) \geq t$. При этом константы $C_1$ и $C_2$ от $t$ не зависят.

% Это нам даёт оценочку $m_{K_4^{(3)-}}(r) \leq r^{3+o(1)}$

% Let $f(n)$ be the minimum possible independence number of $K_{4}^{(3)-}$-free 3-graph.
% It follows from Theorem 1.6 from~\cite{fox2019independent} that
% \begin{equation}
%     f(n) = \Theta\left( \frac{\ln n}{\ln \ln n} \right).
% \end{equation}  
% In paricular, there is a constant $C$ such that for each $n \geq 1$ there is a 3-graph $G_n$ with $V(G_n)=n$ such that
% \begin{equation}
%     \alpha(G_n) \leq C \frac{\ln n}{\ln\ln n}.
% \end{equation}





% В теории Рамсея есть замечательное утверждение: $R_3(K_4^{(3)-},n)\geqslant 2^{cn}$. Его доказательство на самом деле даёт верхнюю оценку и на $m_{K_4^{(3)-}}(r)$, давайте это поймём.

% Рассмотрим случайный турнир (полный орграф) на $v$ вершинах. Построим по нему 3-граф следующим образом: рёбра будут соответствовать треугольникам-циклам. В таком 3-графе нет $K_4^{(3)-}$: если на $4$ вершинах есть два треугольника-цикла, то два других треугольника циклами не являются.

% Остаётся оценить размер независимого множества в этом 3-графе. Независимое множество соответствует транзитивному подтурниру; в самом деле, пусть в независимом множестве есть цикл. Рассмотрим цикл минимальной длины, если его длина больше трех, то любое внутреннее ребро отрезает меньший цикл, противоречие.

% Несложно понять, что найдётся турнир на $v$ вершинах без транзитивных подтурниров размера $c\log v$: вероятность того, что подтурнир на фиксированных $k$ вершинах в случайном турнире транзитивен, не превышает $2^{-ck^2}$, тогда матожидание количества транзитивных подтурниров размера $k>c\log v$ не превосходит
% \[
% \binom{v}{k}\cdot 2^{-ck^2}=2^{ck\log v-ck^2}<1.
% \]

% Итак, нашёлся 3-граф на $v$ вершинах без $K_4^{(3)-}$ с хроматическим числом не меньше $\frac{v}{c\log v}$; в этом графе не более $\binom{v}{3}$ ребер. Взяв $v\sim cr\log r$, получаем 
% \[
% m_{K_4^{(3)-}}(r) \leq cr^3\log^3 r.
% \]


% Совсем недавно это оценку усилили до оптимальной~\cite{fox2019independent}. ПОДРОБНОСТИ ПИСЬМОМ


% \subsection{Верхняя оценочка}

% Я ЗАБЫЛ ПОКАЗАТЕЛЬ У БФМ, ЛЕША, ТЫ СЧИТАЛ.

% В статье~\cite{conlon2010hypergraph} доказывается, что
% \[
% R_3 (4,n) \geq 2^{cn\log n}.
% \]
% То есть, существует 3-граф $H = (V,E)$ без $K_4^{(3)}$, такой что
% \[
% \alpha (H) \leq c\frac{\log |V|}{\log \log |V|}.
% \]
% При $|V| = cr\frac{\log r}{\log \log r}$, мы получаем
% \[
% m_{K_4^{(3)-}}(r) \leq cr^3\left ( \frac{\log r}{\log \log r} \right )^3.
% \]



\subsubsection{The upper bound}
For any $t\geq 1$ there is a $H$-free 3-graph $G_t$ with $|V(G_t)| = t^{At}$ and $\alpha(G_t) < t$.
Put $n = t^{At}$.
For a sufficiently big $t$ we have $A\ln t < t$, so
\begin{equation}
    \frac{\ln n}{\ln \ln n}
    =
    \frac{At \ln t}{\ln (At \ln t)} > \frac{At \ln t}{\ln(t^2)} = \frac{At}{2}.
\end{equation}
Then
\begin{equation}
    \alpha(G_t) < t <
    \frac 2A \cdot 
    \frac{\ln n}{\ln \ln n}.
\end{equation}
Now let us fix a sufficiently big $r$, and let us choose $t$ such that 
\begin{equation}\label{eq:choose_t}
    (t-1)^{A(t-1)} \leq \frac rA \cdot \frac{\ln r}{\ln \ln r} < t^{At}.
\end{equation}
Note that $n = t^{At} > r$ if $r$ is sufficiently big.
Then
\begin{equation}
    \chi(G_t) 
    \geq
    \frac{|V(G_t)|}{\alpha(G_t)}
    >
    \frac{t^{At}}{\frac 2A \cdot \frac{\ln n}{\ln \ln n}}
    >
    r \cdot \left( \frac{\ln r}{\ln \ln r} \biggm/ \frac{\ln n}{\ln \ln n}\right)
    >
    r,
\end{equation}
because $n > r$ and function $\ln x / \ln\ln x$ is increasing when $x > e^e$, which can easily be seen from taking a derivative.
On the other hand,
\begin{equation}
    |E(G_t)|
    <
    \frac {|V(G_t)|^3}{6}
    =
    \frac{t^{3At}}6.
\end{equation}
It is well-known that function $\bigl(\frac t{t-1}\bigr)^t$ is strictly decreasing, so for $t > 2$
\begin{equation}
    t^{3At} < 4^{3A}(t-1)^{3At}.
\end{equation}
Then we have
\begin{equation}
    |E(G_t)| < 
    \frac{4^{3A}}6 \cdot (t-1)^{3At}
    =
    \frac{4^{3A}}6 \cdot \bigl((t-1)^{A(t-1)}\bigr)^{3t/(t-1)}
    \leq
    \frac{4^{3A}}6 \cdot 
        \left(
            \frac rA \cdot \frac{\ln r}{\ln \ln r}
        \right)^{3t/(t-1)},
\end{equation}
which gives us the desired bound.


==> results/trash/orderedRamsey.tex <==
\section{Упорядоченные числа Рамсея}

Надо поглядеть на~\cite{balko2022ordered}.


Пусть $H$, $F$ --- упорядоченные $n$-графы.
\textit{Упорядоченным числом Рамсея} $R_<(H,F)$ называют минимальное число вершин в полном $n$-графе, при любой раскраске которого в синий и красный цвета появляется синяя упорядоченная копия $H$ или красная упорядоченная копия $F$.

 
 
\begin{theorem}[Плухар~\cite{Pl}]
Пусть $H = (V,E)$ --- гиперграф. Следующие утверждения равносильны
\begin{itemize}
    \item $\chi (H) > r$;
    \item для любого порядка $\pi$ на $V$ найдется $\pi$-упорядоченная $r$-цепь.
\end{itemize}
\end{theorem}




\begin{theorem}
Для всех $r > 1$, $t \geq n$ выполняется равенство
\[
R_{<} (P_r, K_t) = (t-1)r + 1.
\]
\end{theorem}

\begin{proof}
Для начала докажем, что в любом гиппогрифе $H = (V,E)$ на $((t-1)r + 1)$-ой вершине найдется либо упорядоченная копия $P_r$ либо $K_t$. Это прямое следствие теоремы Плухара: если $\chi (H) > r$, то обязательно найдется упорядоченная копия $P_r$, если же $\chi(H) \leq r$, то найдется независимое множество размера не менее
\[
\lc\frac{|V(H)|}{r}\rc = \lc\frac{(t-1)r+1}{r}\rc = t.
\]

Теперь приведем пример гиперграфа $H = (V,E)$ на $(t-1)r$ вершинах, обеспечивающего оценку $R_{<} (P_r, K_t) > (t-1)r$.
Рассмотрим разбиение $V$ на непересекающиеся множества $V_1, \dots V_r$ размера $(t-1)$; $E$ состоит из тех и только тех ребер, которые не лежат ни в одном из $V_1, \dots V_r$. Тогда с одной стороны $\alpha (H) = t-1$, с другой стороны $\chi (H) = r$,
что по теореме Плухара гарантирует отсутствие $r$-цепи для хотя бы одного порядка на вершинах.



\end{proof}







==> results/trash/r__4+o_1__.tex <==
\section{Relation with Tur{\'a}n numbers}

Let $\ex(n,F)$ denote the maximum number of edges in an $F$-free 3-graph with $n$ vertices.

\begin{theorem}\label{thm:exnF}
Let $F$ be a 3-graph and let $C_1$ be a constant such that for all $n \geq 1$
\begin{equation}\label{eq:exnF}
    \ex(n,F) \leq C_1n^2.
\end{equation}
Then for any constant $C_2>0$ there exists some $R = R(C_2)$ such that for $r > R$
\begin{equation}\label{eq:r4log}
    m_F(r) > \frac{C_2r^4}{(\ln \ln r)^5}.
\end{equation}
\end{theorem}

\begin{proof}
Let $C_2 > 0$.
Consider a 3-graph $G$ with
\begin{equation}\label{eq:r4t5}
    E(G) \leq \frac{C_2r^4}{(\ln \ln r)^5}.
\end{equation} 
We will show that it is $r$-colorable.
Let $V_0 = V(G)$ and
\begin{equation}
    V_i = 
    \left\{v \in V_{i-1}: 
    \deg_{G[V_{i-1}]} v \geq \frac1{C_3}\left(\frac{r}{\ln \ln r} \right )^2 \right\},
    \quad
    i \geq 1,
\end{equation}
where $C_3$ is chosen to satisfy inequality
\begin{equation}
    \frac 1{C_3}
    \left(
        \frac{r}{\ln\ln r}
    \right)^2
    \leq
    \frac 1{3e}
    \left[
        \frac{r}{\log_2\ln r}
    \right]^2
\end{equation}
% \begin{equation}
%     \left\lceil
%     \sqrt{
%         e\left(
%             \frac 1{C_3}
%             \left(
%                 \frac r{\ln \ln r}
%             \right)^2
%         + 1
%         \right)
%     }\,\,
%     \right\rceil
%     = r_1 \leq
%     \frac{r}{\log_2 \ln r},
% \end{equation}
for, let's say, $r > 100$,
so by Lemma~\ref{lm:3graph-coloring} every 3-graph $G[V_i \setminus V_{i+1}]$ for $i\geq 0$ has a proper coloring in $\bigl[\frac{r}{\log_2\ln r}\bigr]$ colors. Clearly, $C_3$ can be chosen independently of $r$.

Now we going to estimate sizes of $E(G[V_i])$ and $V_{i+1}$ from above for each $i \geq 0$.
As $V_{i+1} \subset V_i$, we have
\begin{equation}
    \# E(G[V_i]) \geq
    \frac 13 \sum_{v \in V_{i+1}} \deg_{G[V_i]} v
    \geq 
    \frac 13 \cdot \# V_{i+1} \cdot 
        \frac 1{C_3}
        \left(
            \frac{r}{\ln \ln r}
        \right)^2,
\end{equation}
so
\begin{equation}
    \label{eq:v_bound}
    \# V_{i+1} \leq 3C_3 
        \left(
            \frac{\ln \ln r}{r}
        \right)^2
        \# E(G[V_i]).
\end{equation}
Also we have bound~\eqref{eq:r4t5} for $\#E(G[V_0])$ and by~\eqref{eq:exnF}
\begin{equation}
    \label{eq:e_bound}
    \#E(G[V_i]) \leq C_1 (\#V_i)^2 \ \text{for $i \geq 1$}.
\end{equation}
 Put $C = C_1C_2(3C_3)^2$.
Combining~\eqref{eq:e_bound} and~\eqref{eq:v_bound} and using induction on $i$, we obtain for $i\geq0$ 
\begin{equation}\label{eq:egvi_bound}
    \# E(G[V_{i}]) \leq 
        \frac{C^{2^i}}{C_1\cdot (3C_3)^2}
        % C_1^{2^i-1} \cdot C_2^{2^i} \cdot
        % (3{C_3})^{2^{i+1}-2} 
        \cdot
        \frac{r^4}{(\ln \ln r)^{2^{i}+4}},
\end{equation}
\begin{equation}\label{eq:vi_bound}
    \# V_{i+1} \leq 
        \frac{C^{2^i}}{C_1\cdot 3C_3}
        % C_1^{2^i-1} \cdot C_2^{2^i} \cdot 
        %  (3{C_3})^{2^{i+1}-1}  
        \cdot
         \frac{r^2}{(\ln \ln r)^{2^i + 2}}.
\end{equation}
The last inequality implies $V_N = \emptyset$ for $N \geq \log_2 \ln r + 1$ and large enough $r$. 
Indeed, for $r \geq r_0(C_1,C_3)$
\begin{equation}
    \# V_{N} 
    \leq
        \frac{C^{2^{N-1}}}{C_1\cdot 3C_3}
        % C_1^{2^i-1} \cdot C_2^{2^i} \cdot 
        %  (3{C_3})^{2^{i+1}-1}  
        \cdot
        \frac{r^2}{(\ln \ln r)^{2^{N-1} + 2}}
    \leq
        \frac{r^2}{C_1\cdot 3C_3 \cdot(\ln \ln r)^2}
        \bigg/
        \left(
            \frac{\ln \ln r}{C}
        \right)^{2^{N-1}}
        \leq
        r^2 \bigg/
        \left(
            \frac{\ln \ln r}{C}
        \right)^{\ln r}
        =
        \left(
            \frac{Ce^2}
            {\ln \ln r}
        \right)^{\ln r}
    % C_0^{2^{N-1}-1} \cdot C^{2^{N-1}} \cdot 
    %      (3{C_1})^{2^N-1} \cdot \frac{r^2}{(\ln \ln r)^{2^{N-1} + 2}}
    % \leq
    % r^2\biggm/\left(
    %     \frac{\ln \ln r}{C_0 \cdot C \cdot (3C_3)^2}
    % \right)^{2^{N-1}}
    % =
    % r^2\biggm/\left(
    %     \frac{\ln \ln r}{C_2}
    % \right)^{\ln r}
\end{equation}
which is less than 1 when $\ln \ln r > Ce^2$, which is
\begin{equation}
    r > e^{e^{Ce^2}}.
\end{equation}
We divided $V$ in at most $\log_2 \ln r$ sets of form $V_i\setminus V_{i+1}$, and each 3-graph $G[V_i\setminus V_{i+1}]$ has a proper coloring with at most $\frac r{\log_2\ln r}$ colors, so $G$ is $r$-colorable. Therefore we can put $R = \max(100, r_0, e^{e^{Ce^2}})$. 
\end{proof}



\section{More examples}

\begin{proposition}\label{pr:edges_ordering}
Let $H$ be a 3-graph, such that $t=|V(H)|=|E(H)|+2$. Suppose that there is an ordering of edges  $e_1,\dots,e_{t-2}$, that for each $i>1$ $e_i=\{a_i,b_i,c_i\}$, where $\{a_i,b_i\}\subset e_{j(i)}$ for some ${j(i)}<i$ and $c_i\not\in e_j$ for $j<i$. Then 
\begin{equation}    
    ex(n,H)\leqslant (t-3)\binom{n}{2}.
\end{equation}
\end{proposition}
\begin{proof}
Suppose that 3-graph $G$ has more than $(t-3)\binom n2$ edges. 
We show that some subgraph of $G$ is isomorphic to $H$.

Let us repeat the following procedure: if there is an edge $e = {v_1,v_2,v_3}$ such that the pair $(v_1,v_2)$ is contained in at most $t-3$ edges (including $e$), remove $e$.
There will be removed at most $(t-3)\binom{n}{2}$ edges, and each pair of vertices will be joined by either 0 or at least $t-2$ edges. Denote resulting 3-graph by $G'$.

Let $H_i$ be a subgraph $H$ induced by edges $e_1,\dots,e_i$.
We removed at most $(t-3)\binom{n}{2}$ edges from $G$, so $\# E(G') \geq 1$. Subgraph of $G'$ induced by one edge is isomorpic to $H_1$. Now we show that if there is a subgraph $H \subset G'$ isomorphic to $H_{i-1}$ then there is a subgraph isomorphic to $H_{i}$. All we have to do is find an edge which can be put in correspondence to $e_i$.
$H_{i-1}$ has an edge $e_{j(i)} \supset \{a_i, b_i\}$. Consider $v,u \in V(H)$ that correspond to $a_i$ and $b_i$. There is an edge in $H$ that corresponds to $e_{j(i)}$, so $v$ and $u$ are joined by at least $t-2$ edges. We have $\# E(H) = \#E(H_{i-1}) = i-1 < t-2$, so there is $e \in E(G')\setminus E(H)$ which contains $v$ and $u$, and it can be put in correspondence to $e_i$.

So there is subgraph of $G'$ that is isomorphic to $H_{i-2} = H$ and since $G'\subset G$, it is a subgraph of $G$.
% Будем последовательно находить копию $H_i$: если уже есть копия $H_{i-1}$, то возьмём в ней ребро, соответствующее $e_{j(i)}$. Оно проходит через пару вершин, соответствующих $\{a_i,b_i\}$. Тогда через эту пару вершин проходит хотя бы $t-2$ ребра, в частности, одно из этих рёбер проходит через вершину, не лежащую в копии $H_{i-1}$ (так как $|V(H_{i-1})|<t$). Это ребро вместе с копией $H_{i-1}$ образует копию $H_i$.
\end{proof}

Recall that a $k$-graph $G$ with at least two edges is called \textit{balanced} if 
\begin{equation}\label{eq:balance}
    \max_{G' \subset G}
    \frac{E(G')-1}{V(G')-k}
    =
    \frac{E(G)-1}{V(G)-k},
\end{equation}
where maximum is taken over all subgraphs $G'$ of $G$ with at least two edges. The number~\eqref{eq:balance} is called \textit{the balance} of $G$.

\begin{corollary}
    Suppose that 3-graph $H$ satisfies the conditions of Proposition~\ref{pr:edges_ordering}. Then for some positive constants $C_1$ and $C_2$ and for sufficiently large $r$ 
    \begin{equation}
        C_1 \frac{r^4}{(\ln \ln r)^5} < m_H(r) < C_2 r^4 (\ln r)^2.
    \end{equation}
\end{corollary}
\begin{proof}
    By Proposition~\ref{pr:edges_ordering} such $H$ satisfies the conditions of Theorem~\ref{thm:exnH}, so lower bound holds.
    
    Note that $E(F) \leq V(F)+2$ for any subgraph $F$ of $H$, so $H$ is balanced with the balance $\frac{E(H)-1}{V(H)-3} = 1$. By Theorem~\ref{thm:bohman2010-4} with $\rho = 1$ we obtain the upper bound.
\end{proof}

% Таким образом, для любого графа, удовлетворяющего условию предложения, верна показанная выше оценка 
% \[
% m_H(r) > c_H \frac{r^4}{(\ln \ln r)^5}.
% \]

% С другой стороны, несложно заметить, что в любом подграфе $G$ графа $F$ выполняется неравенство $E(G)\leqslant V(G)+2$, то есть $F$~--- балансный с балансом $\frac{E(H)-1}{V(H)-3}=1$. Тогда из теоремы 4 в~\cite{bohman2010coloring} следует, что $m_H(r) < C_Hr^4\log^2 r$.











